Linear Set Reconciliation with $O(d)$ Additive Redundancy

In set reconciliation, two parties holding sets $A, B \subseteq [n]$ with $|A \triangle B| \le d$ seek to recover their symmetric difference from short $\mathbb{F}_2$-linear sketches, which is equivalent to recovering a $d$-sparse vector $x = \mathbf{1}_{A \triangle B} \in \mathbb{F}_2^n$ from its syndrome $Hx \in \mathbb{F}_2^m$. While the information-theoretic counting bound requires $L(n,d) := \log \sum_{i=0}^d \binom{n}{i} = d\log(n/d) + \Theta(d)$ bits, existing polynomial-time schemes either use at least $d\lceil\log(n+1)\rceil$ bits (algebraic sketches, leaving an $\Omega(d\log d)$-bit gap) or incur a multiplicative $(1+\delta)L(n,d)$ overhead (peeling-based sketches), raising the question of whether $L(n,d) + O(d)$ bits is achievable with fast updates and decoding. We construct a public-coin randomized $\mathbb{F}_2$-linear sketch of length $L(n,d) + O(d) + \lambda\log^{O(1)} n$ that recovers each fixed input of weight at most $d$ with probability at least $1 - 2^{-\lambda}$, with $\log^{O(1)} n$ update time and $d\exp(O((\log\log n)^2)) = dn^{o(1)}$ worst-case decoding time. In particular, for $n \le 2^{\operatorname{polylog}(d)}$ and $\lambda \le d^{1-\Omega(1)}$, this achieves $L(n,d) + O(d)$ bits with $\operatorname{polylog}(d)$ update time and $d^{1+o(1)}$ decoding time. Our construction encodes $d$ permuted rows via randomly scaled Pinsketch syndromes and sketches the resulting bit array column by column. Decoding columns sequentially from prefix predictions cancels recovered rows and exposes undecided rows as decoder-side hints, reducing each column to a hinted sparse recovery problem that we solve via a recursive sketch, HintSketch.

==> 2609-version/ai-revision-format.tex <==
%
\makeatletter
\@for\ai@key:=MTZ03,GM11,HPW23,BKW24,FLOS24,KPW26,Hae19,GSTV07,XYZ26,PBS20,YGA24,MBYR23,KYR25,Wal25,KRU11,Ari09,Ari10,Ber70,Str12\do{%
  \expandafter\def\csname ai@bib@\ai@key\endcsname{1}}
\@for\ai@key:=EGUV11,Graphene19,LossRadar16,ChameleMon23\do{%
  \expandafter\def\csname ai@newbib@\ai@key\endcsname{1}}
\newcommand{\ai@bibitem}[2][]{%
  \edrev%
  \if\relax\detokenize{#1}\relax
    \ai@originalbibitem{#2}%
  \else
    \ai@originalbibitem[#1]{#2}%
  \fi}
\AddToHook{env/thebibliography/begin}{%
  \let\ai@originalbibitem\bibitem
  \let\bibitem\ai@bibitem}
\AddToHook{env/thebibliography/end}{\edrev}
\makeatother

